Re-purposing Heterogeneous Generative Ensembles with Evolutionary Computation

Generative Adversarial Networks (GANs) are popular tools for generative modeling. The dynamics of their adversarial learning give rise to convergence pathologies during training such as mode and discriminator collapse. In machine learning, ensembles of predictors demonstrate better results than a single predictor for many tasks. In this study, we apply two evolutionary algorithms (EAs) to create ensembles to re-purpose generative models, i.e., given a set of heterogeneous generators that were optimized for one objective (e.g., minimize Frechet Inception Distance), create ensembles of them for optimizing a different objective (e.g., maximize the diversity of the generated samples). The first method is restricted by the exact size of the ensemble and the second method only restricts the upper bound of the ensemble size. Experimental analysis on the MNIST image benchmark demonstrates that both EA ensembles creation methods can re-purpose the models, without reducing their original functionality. The EA-based demonstrate significantly better performance compared to other heuristic-based methods. When comparing both evolutionary, the one with only an upper size bound on the ensemble size is the best.

==> conclusion.tex <==
\section{Conclusion \& Future Work}
\label{sec:conclusion}

In this paper, we have investigated how population diversity as
employed by spatial coevolutionary (in particular competitive)
algorithms as an option to enhance the performance of gradient-based
GAN training methods. We presented \horse, a framework that combines
the advantages of gradient-based optimization for GANs with those of
coevolutionary systems, and allows scaling over a distributed spatial
grid topology. Using a relatively small spatial grid is sufficient to
overcome the common limitations of GANs, due to the spatial grid and
asynchronous evaluation. The performance can improve with increased
grid size. In addition, \horse scales well up to the grid sizes
elaborated in the conducted experiments (i.e. a grid size of six by
six). We enhanced an existing spatial evolutionary GAN training
framework that promoted genomic diversity by probabilistically
choosing one of three loss functions. This method, called \SEGAN was
tested on the MNIST and CelebA data sets showed no drop in performance
and high diversity in label space, as well as on the TVD measure.

Future work will include the evaluation on more data sets and longer
training epochs. In addition, even better results may be achieved by
including improved GAN types like the recently introduced
WGAN~\cite{arjovsky2017wasserstein}. More heterogeneous cell
configurations, i.e. architectures and data slices can also be
explored. Furthermore, the constants in the computational complexity
of \horse could be reduced. Finally, other advancements in
evolutionary algorithms that can improve the robustness of GAN
training, e.g. temporal evolutionary training, need to be considered.


==> experiments.tex <==
\section{Experimental Setup}
\label{sec:experimental-setup}

The MNIST image dataset is used to asses the generative modeling
performance. This dataset \cite{lecun1998mnist} has been widely used,
and is appropriate for investigating mode collapse due to its limited
target space (namely the digits from zero to nine).  This
experimental analysis compares: \pagan, \spagan, \nocommgan, and
\Lipi.

The communication among the neighborhoods is affected by the grid
size~\cite{schmiedlechner2018lipizzaner}. We evaluate \spagan and
\Lipi by using three different grid sizes: \xGrid{3}, \xGrid{4}, and
\xGrid{5}, in order to asses the impact of this parameter.

The assessment of the quality of the generated data is done by
evaluating the \textbf{FID} score.  The \textbf{network diversity} of
the trained models is evaluated by the $L_2$ distance between the
parameters of the generators.  The \textbf{total variation distance
  (TVD)}~\cite{li2017distributional}, is a scalar that measures class
balance, is used to analyze the diversity of the generated data
(Eq.~\ref{eq:tvd}).

\begin{equation}
\small
TVD = \frac{1}{2}\sum_{c \in Classes}{\mid freq(real_c) - freq(fake_c) \mid}
\label{eq:tvd}
\end{equation}
%
TVD reports the difference between the proportion of the generated
samples of a given digit and the ideal proportion (10\% in MNIST).
The TVD is measured by generating 50,000 images (digits) of the best
ensemble of generators for the different methods and grid sizes in
the 30~independent runs. Note that even though FID score performs well
in terms of discriminability and robustness when dealing with image
data, it lacks capacity to represent the diversity of the samples
generated~\cite{BORJI201941}. This justifies analyzing the output
diversity individually. Finally, the \textbf{computational cost} is
measured in run time.  Note that we use cloud architecture, which could
generate some variance in terms of computational efficiency
results. In order to allow comparisons between the analyzed methods,
we use the same computation platform for each grid size. All
implementations use the same \texttt{Python} libraries and versions.
The distribution of the results are not Gaussian, so a Mann-Whitney U
statistical test is applied to evaluate their significance.

The methods evaluated here are configured according to the settings
proposed by the authors of \Lipi~\cite{schmiedlechner2018lipizzaner}. %They have been implemented in \texttt{Python3} and \texttt{pytorch}\footnote{Pytorch Website - \texttt{https://pytorch.es/}}.  
The experimental analysis is performed on a cloud computation platform that provides 8~Intel Xeon cores 2.2GHz with 32 GB RAM and a NVIDIA Tesla P100 GPU with 16 GB RAM.

%\begin{table}
%  \centering
%  \caption{Setup for experiments conducted.}
%  \label{tbl:exp-lpz}
%  \small
%
%  \begin{tabular}{ll}
%				\hline
%\textbf{Parameter} & \textbf{Value} \\
%		\hline
%		\multicolumn{2}{c}{\textit{Coevolutionary settings}} \\ 
%		Generations & 200  \\
%                % TODO mark up clearer when 20 generations for CelebA is run
%		Population size per cell & 1 \\ 
%		Tournament size & 2 \\ 
%		Grid size & \xGrid{3}, \xGrid{4}, \xGrid{5} \\
%		Mixture mutation scale & 0.01  \\ 
%		\multicolumn{2}{c}{\textit{Hyperparameter mutation}} \\ 
%		Optimizer & Adam \\ 
%		Initial learning rate & 0.0002 \\ 
%		Mutation rate & 0.0001   \\ 
%		Mutation probability & 0.5 \\ 
%                \multicolumn{2}{c}{\textit{Network topology}} \\ 
%		Network type  & MLP  \\ 
%		Input neurons & 64 \\ 
%		Number of hidden layers & 2 \\ 
%		Neurons per hidden layer & 256  \\ 
%		Output neurons  & 784  \\ 
%		Activation function & $tanh$\\ 
%		\multicolumn{2}{c}{\textit{Training settings}} \\ 
%		Batch size  & 100 \\ 
%				\hline
%	\end{tabular}
%\end{table}
%



\section{Results and Discussion}
\label{sec:results}

%% TODO restate the RQ and hypothesis

This section discusses the main results of the experiments carried out
to evaluate \pagan, \nocommgan, \spagan, and \Lipi.


\noindent
\begin{figure*}
\begin{minipage}[!h]{0.32\textwidth}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{images/extended-selection-vs-no_selection-9-boxplot}
\caption{Boxplot that shows the best FID from \spagan and \Lipi in each independent run for each grid size.}\label{fig:fid-gridsize-boxplot}
\end{figure}
\end{minipage}
\hspace{0.1cm}
\begin{minipage}[!h]{0.32\textwidth}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{images/fid-evolution-gap-mnist-9-pagan}
\caption{Median FID evolution through the 200 epochs (\xGrid{3}-Grid).}\label{fig:fid-gridsize-evolution}
\end{figure}
\end{minipage}
\hspace{0.1cm}
\begin{minipage}[!h]{0.32\textwidth}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{images/fid-evolution-mnist-differences}
\caption{Differences between the FID at a given epoch when using \xGrid{3} and \xGrid{4} or \xGrid{5} ($diff\_FID^{s \times s}_{i}$).}\label{fig:fid-differences}
\end{figure}
\end{minipage}
\end{figure*}


\subsection{Generator Quality}
\label{sec:final-fid}

Table~\ref{tab:final-fids} summarizes the results by showing the best
FID scores for the different methods and grid sizes in the
30~independent runs.

\begin{table}[!h]
	\centering
	\small
	\caption{\small FID results for \textit{MNIST} experiments.}
	\label{tab:final-fids}
\begin{tabular}{lrrrrr}
\toprule
\textbf{Method} &  \textbf{Mean}$\pm$\textbf{Std} &  \textbf{Median} &   \textbf{Iqr} &   \textbf{Min} &   \textbf{Max} \\
\midrule
\multicolumn{6}{c}{\textit{\xGrid{3}-Grid}} \\
\oppagan & 51.15$\pm$14.06 & 46.85 &  6.40 &  40.81  &  112.58 \\ 
\spagan & 43.59$\pm$5.53 & 43.09 &  5.94 &  30.65  &  51.81 \\ 
\nocommgan & 881.79$\pm$52.67 & 871.04 &  66.81 &  798.03  &  998.79 \\ 
\Lipi & 40.93$\pm$8.51 & 39.44 &  10.59 &  28.04  &  62.10 \\ 
\midrule
\multicolumn{6}{c}{\textit{\xGrid{4}-Grid}} \\
\spagan & 37.97$\pm$8.89 & 35.98 &  13.61 &  23.69  &  56.36 \\ 
\Lipi & 32.84$\pm$6.93 & 32.22 &  7.23 &  19.15  &  46.53 \\
\midrule
\multicolumn{6}{c}{\textit{\xGrid{5}-Grid}} \\
\spagan  & 39.11$\pm$4.00 & 39.61 &  5.29 &  27.39  &  48.03 \\ 
\Lipi & 28.74$\pm$4.91 & 28.14 &  7.45 &  22.56  &  40.57 \\
\bottomrule
\end{tabular}
\end{table}

As shown in Table~\ref{tab:final-fids}, \Lipi obtains the lowest/best
\textbf{Mean}, \textbf{Median}, and \textbf{Min} FID scores for all
grid sizes.  \spagan and \pagan are the second and third best methods,
respectively.  \nocommgan presents the lowest quality by showing the
highest (worst) FID scores.  The FID values in terms of hundreds
indicate that the generators trained with this method are not capable
of creating adequate MNIST data samples. The Mann-Whitney U shows that
the methods that exchange individuals among the neighborhoods, i.e.,
\Lipi and \spagan, are significantly better than \pagan and \nocommgan
($\alpha<<0.001$). These results are confirmed by posthoc statistical
analysis.  According to this analysis there is not statistical
difference between \Lipi-\xGrid{3} and \spagan for all evaluated grid
sizes.  In turn, \Lipi run in a \xGrid{4} and \xGrid{5} outperform all
the other methods and \Lipi \xGrid{5} provides the generators with
highest quality.  

\nocommgan does not converges since the individuals of one
sub-population are evaluated against individuals of the other
sub-population that are randomly chosen. As the accuracy of their
fitness evaluation depends subjectively on the quality of the randomly
chosen opponent, it is likely that the fitness value does not
correspond to the real quality of the individual, and therefore, the
selection/replacement operator does not promote the objectively best
solution in the sub-population. Then, the \textit{center} of the cell
is updated with not the best pair generator-discriminator.

The boxplot in Figure~\ref{fig:fid-gridsize-boxplot} shows the FID
results of \spagan and \Lipi with different grid sizes. This figure
allows the comparison of the FID results of \spagan and \Lipi changing
the grid sizes.  For all grid sizes, \spagan provides worse quality
than \Lipi (higher FIDs).  \spagan has similar quality for all grid
sizes, but \Lipi improves when the grid size is increased.  Thus, the
larger the grid size, the greater the difference between these two
methods.  Thus, we observe the benefits of increasing the diversity
(population/grid size) when applying the coevolutionary approach with
selection and replacement of \Lipi. The results of \Lipi are mainly
due to, first, the larger population size ability to encompass a
higher diversity, and second, the selection/replacement process
applied by the coevolutionary training method by \Lipi accelerates the
convergence of the population to higher quality generators.

\begin{figure*}[h!]
\centering
\subfloat[\scriptsize{\spagan(25)}]
         {\includegraphics[width=0.12\textwidth]{images/SPaGAN-025.pdf}\label{fig:heatmpa-mnist-4x4-025-unif}}\hspace{0.cm}
\subfloat[\scriptsize{\spagan(50)}]
         {\includegraphics[width=0.12\textwidth]{images/SPaGAN-050.pdf}\label{fig:heatmpa-mnist-4x4-050-unif}}\hspace{0.cm}
\subfloat[\scriptsize{\spagan(75)}]
         {\includegraphics[width=0.12\textwidth]{images/SPaGAN-075.pdf}\label{fig:heatmpa-mnist-4x4-075-unif}}\hspace{0.cm}
\subfloat[\scriptsize{\spagan(100)}]
         {\includegraphics[width=0.12\textwidth]{images/SPaGAN-100.pdf}\label{fig:heatmpa-mnist-4x4-100-unif}}
\hspace{0.cm}
\subfloat[\scriptsize{\Lipi(25)}]
         {\includegraphics[width=0.12\textwidth]{images/Lipi-025.pdf}\label{fig:heatmpa-mnist-4x4-025-op}}\hspace{0.cm}
\subfloat[\scriptsize{\Lipi(50)}]
         {\includegraphics[width=0.12\textwidth]{images/Lipi-050.pdf}\label{fig:heatmpa-mnist-4x4-050-op}}\hspace{0.cm}
\subfloat[\scriptsize{\Lipi(75)}]
         {\includegraphics[width=0.12\textwidth]{images/Lipi-075.pdf}\label{fig:heatmpa-mnist-4x4-075-op}}\hspace{0.cm}
\subfloat[\scriptsize{\Lipi(100)}]
         {\includegraphics[width=0.12\textwidth]{images/Lipi-100.pdf}\label{fig:heatmpa-mnist-4x4-100-op}}

        \caption{\small{FID score distribution through the grid at different epochs (expresed between parentesis) of an independent run for \spagan and \Lipi in a \xGrid{4} grid. Lighter blues represent lower (better) FID scores. }} 
  \label{fig:fids-in-grid}
\end{figure*}

\subsection{Quality (FID) Evolution}
\label{sec:fid-evolution}

Figure~\ref{fig:fid-gridsize-evolution} shows the evolution of the
median FID over each training epoch when using \pagan, \spagan, and
\Lipi and \spagan when using \xGrid{3} grid (population of 9)
Figure~\ref{fig:fid-differences} illustrates the differences between
the FID score when using \xGrid{3} and \xGrid{4} or \xGrid{5} for the
same method.  This difference for the grid size \xGrid{s} at the $i$
epoch is computed as \hbox{$diff\_FID^{s \times s}_{i}=FID^{3\times
    3}_{i} - FID^{s \times s}_{i}$}.  This figure allows to evaluate
the impact on the FID evolution when using different grid (population)
sizes.

According to Figure~\ref{fig:fid-gridsize-evolution}, \Lipi is able to
improve the performance of the generators ensemble faster than \spagan
(during the early epochs). This is also illustrated by
Figure~\ref{fig:fids-in-grid} that shows the FID scores in the grid of
a given independent run at the epoch number 25, 50, 75, and 100.  This
is mainly due to the capacity of exploitation of this method when
using the selection/replacement process.  After the first 75 to 100
training epochs, the FID does not show such a reduction in \Lipi , but
\spagan is able to keep reducing it until the end of the training
process.  \pagan also shows fast FID reduction at the begining of the
training process. However, the FID sharply oscillates during the first
75 iterations.  Finally, \pagan converges to higher FID scores than
\Lipi and \spagan.

When comparing the two best training methods,
Figure~\ref{fig:fid-differences} shows how \Lipi provides lower FIDs
and it is able to converge faster as the grid size increases during
the first iterations.  In contrast, \spagan gets better FIDs when
increasing the grid size only during the first 50 epochs. \Lipi is
able to take advantage of the diversity generated when the grid size
increase to converge faster to lower FIDs than \spagan.  Thus, in
terms of convergence, selection/replacement helps convergence of the
coevolutionary training method when exchanging information (solutions)
with the neighborhoods.

\subsection{Generator Output Diversity} 
\label{sec:tvd}

The output diversity reports the class distribution of the fake data
produced by a generative model. As we are addressing the MNIST
problem, the ability of creating digits from 0 to 9 is
evaluated. Table~\ref{tab:final-tvds} summarizes the results.

\begin{table}[!h]
	\centering
	\small
	\caption{\small TVD results for \textit{MNIST} experiments (Low TVD indicates more diversity).}
	\label{tab:final-tvds}
\begin{tabular}{lrrrrr}
\toprule
\textbf{Method} &  \textbf{Mean}$\pm$\textbf{Std} &  \textbf{Median} &   \textbf{Iqr} &   \textbf{Min} &   \textbf{Max} \\
\midrule
\multicolumn{6}{c}{\textit{\xGrid{3}-Grid}} \\
\oppagan & 0.14$\pm$0.02 & 0.14 &  0.04 &  0.10  &  0.19 \\ 
\spagan & 0.12$\pm$0.02 & 0.12 &  0.02 &  0.08  &  0.16 \\  
\nocommgan & 0.83$\pm$0.08 & 0.82 &  0.14 &  0.69  &  0.91 \\ 
\Lipi & 0.12$\pm$0.03 & 0.12 &  0.04 &  0.08  &  0.18 \\ 
\midrule
\multicolumn{6}{c}{\textit{\xGrid{4}-Grid}} \\
\spagan & 0.12$\pm$0.02 & 0.12 &  0.03 &  0.08  &  0.16 \\ 
\Lipi & 0.11$\pm$0.02 & 0.11 &  0.02 &  0.05  &  0.16 \\ 
\midrule
\multicolumn{6}{c}{\textit{\xGrid{5}-Grid}} \\
\spagan  & 0.11$\pm$0.02 & 0.11 &  0.03 &  0.07  &  0.15 \\ 
\Lipi & 0.10$\pm$0.02 & 0.11 &  0.02 &  0.06  &  0.16 \\ 
\bottomrule
\end{tabular}
\end{table}

For the \xGrid{3} grid experiments, a similar behaviour is observed to
that seen in FID score.  \nocommgan shows the worst (high) TVD values.
\pagan is computes competitive TVDs but it is statistically less
competitive than \spagan and \Lipi according to the Mann-Whitney U
test.  \spagan and \Lipi provide the best results obtaining the same
\textbf{Mean}, \textbf{Median}, and \textbf{Min} values (there are not
statistical difference between them).  Therefore, when using
communication between the neighborhoods during the training, the
generators are able to produce more diverse data samples.

When increasing the grid size, \spagan and \Lipi improve their results
(see Table~\ref{tab:final-tvds}).  However, \spagan does not
show statistical differences between the same algorithm with different
grid sizes.  When \Lipi uses
a \xGrid{5} grid provides statistically better results than the same
algorithm in \xGrid{3} grid and than \spagan in \xGrid{3} and \xGrid{4}
grids. The coevolutionary approach used in \Lipi takes advantage of
the diversity generated when increasing the grid size to train
generators that creates more diverse data samples.

According to these results and the ones in Section~\ref{sec:final-fid}, we can answer \textbf{RQ1:} \textit{What is the effect on the quality of the generators  when the training is given with communication or isolation and presence or absence of selection pressure?} 
The samples generated by \Lipi are the ones with more quality and they are the more diverse ones, this is mainly due to the algorithm is able to converge to better solutions. 
The methods that exchange individuals (\Lipi and \spagan) are the ones ended with better quality generators. 
Isolation in training converged to good solutions when the cell was optimizing only one GAN (\pagan). However, when isolation is coupled with a sub-population that applies selection pressure the algorithm was not able to converge, and therefore, the quality of the generators returned is the worst. 


\subsection{Genome Space Diversity}

We investigate the diversity of the parameters of the evolved networks
(genome space) to see if one network is duplicated over the entire
grid and neighborhoods.  Table~\ref{tab:MNIST_diversity} summarizes
the results of evaluating the $L_2$ distance for the population at the
end of the independent run that returned the median FID.  The heatmap
in Figure~\ref{fig:MNIST_diversity} shows the $L_2$ distances between
all the cells in the grid (x and y axes are the cell number).

\begin{table}[!h]
	\centering
	\small
	\caption{\small Diversity of population (whole grid) in \textit{genome} space. $L_2$ distances  between the generators in the population on MNIST at the final generation.}
	\label{tab:MNIST_diversity}
\begin{tabular}{lrrrrr}
\toprule
\textbf{Method} &  \textbf{Mean}$\pm$\textbf{Std} &  \textbf{Median} &   \textbf{Iqr} &   \textbf{Min} &   \textbf{Max} \\
\midrule
\multicolumn{6}{c}{\textit{\xGrid{3}-Grid}} \\
\oppagan & 109.98$\pm$41.15 & 128.26 &  27.89 &  90.82  &  138.02 \\ 
\spagan & 72.70$\pm$25.75 & 81.72 &  2.66 &  78.32  &  84.82 \\
\nocommgan & 71.07$\pm$25.29 & 79.42 &  5.67 &  74.00  &  86.01 \\ 
\Lipi & 13.85$\pm$8.29 & 18.06 &  15.32 &  4.09  &  23.46 \\ 
\midrule
\multicolumn{6}{c}{\textit{\xGrid{4}-Grid}} \\
\spagan & 87.90$\pm$22.71 & 93.75 &  1.36 &  91.44  &  95.95 \\ 
\Lipi & 30.99$\pm$24.28 & 38.09 &  55.82 &  2.72  &  61.34 \\ 
\midrule
\multicolumn{6}{c}{\textit{\xGrid{5}-Grid}} \\
\spagan  & 87.96$\pm$18.06 & 91.60 &  3.30 &  87.22  &  96.87 \\ 
\Lipi & 31.98$\pm$15.31 & 36.71 &  21.32 &  4.28  &  52.14 \\ 
\bottomrule
\end{tabular}
\end{table}


These results for generators show that there is no duplication of
networks when observing the generator population.  The highest
generators diversity is shown by \pagan. This is due to this method
trains a single generator against a single discriminator and it does
not use any type of information exchange or communication during the
training process.

When comparing between the spatially distributed methods, \spagan and
\nocommgan provide networks with similar $L_2$ distances in \xGrid{3}
grid, which in turn it is higher than the diversity provided by \Lipi.
This is mainly due to the combination of both communication and the
application selection/replacement on the sub-populations applied by
\Lipi provokes the sub-populations converge to similar accurate
individuals, limiting the diversity.

The genome diversity in \Lipi is increased when increasing the size of
the grid (see in Figure~\ref{fig:MNIST_diversity} how the heatmap gets
darker as the grid size is larger).  \spagan increases the $L_2$
distances with the grid size but in a lower proportion, e.g., from
\xGrid{3} to \xGrid{4} \Lipi increases in 123.75\% and \spagan in
20.90\%. The diversity in the genome space helps the creation of
ensembles that are able to provide better accuracy. For this reason,
\Lipi can improve results with an increasing grid size (and
diversity).

\begin{figure*}[!h]
\centering
  \subfloat[\scriptsize{\pagan(\xGrid{3})}]
         {\includegraphics[width=0.12\textwidth]{images/minst-9-no-cooperative}\label{fig:mnist-nets-3x3-pagan}}
         \subfloat[\scriptsize{\nocommgan(\xGrid{3})}]
         {\includegraphics[width=0.12\textwidth]{images/mnist-9-no-selection-d}\label{fig:mnist-nets-3x3-nocomgan}}  
         \subfloat[\scriptsize{\spagan(\xGrid{3})}]
         {\includegraphics[width=0.12\textwidth]{images/mnist-9-no-selection-d}\label{fig:mnist-nets-3x3-pagan}}
    \subfloat[\scriptsize{\Lipi(\xGrid{3})}]
         {\includegraphics[width=0.12\textwidth]{images/mnist-9-selection-b}\label{fig:mnist-nets-3x3-lipi}} 
	     \subfloat[\scriptsize{\spagan(\xGrid{4})}]
         {\includegraphics[width=0.12\textwidth]{images/4x4-no-sel-1}\label{fig:mnist-nets-4x4-pagan}}
         \subfloat[\scriptsize{\Lipi(\xGrid{4})}]
         {\includegraphics[width=0.12\textwidth]{images/mnist-16-selection-1}\label{fig:mnist-nets-4x4-lipi}}
             \subfloat[\scriptsize{\spagan\xGrid{5}}]
         {\includegraphics[width=0.12\textwidth]{images/5x5-no-sel-1}\label{fig:mnist-nets-5x5-pagan}}
    \subfloat[\scriptsize{\Lipi(\xGrid{5})}]
         {\includegraphics[width=0.12\textwidth]{images/5x5-sel-2}\label{fig:mnist-nets-5x5-lipi}}
        \caption{\small{Diversity of population in
            \textit{genome} space. Heatmap of $L_2$ distance between
            the generators in the population on MNIST at
            the final generation. Dark indicates small distance. }}
  \label{fig:MNIST_diversity}
\end{figure*}

Answering
\textbf{RQ2:} \textit{What is the effect on the genome space (parameters/weights of the networks) when applying or not communication among the neighborhoods and using or not selection/replacement operator?} 
The combination of communication and selection pressure provokes \Lipi to converge to similar high quality generators. 
Complete isolation and no-population based GAN training (\pagan) converges to highly different generators, which is expected. 
\spagan illustrates how the absence of selection pressure in the populations keep the individuals diverse in the grid, even there is communication. 
In \xGrid{3} grid experiments, \nocommgan and \spagan has similar diversity but highly different quality. This shows how keeping diversity is not enough to ensure robust GAN training. 




\subsection{Computational Efficiency}

Now, we analyze the computational efficiency of the GAN training
methods, taking into account that they applied the same number of
training epochs but using different types of strategies.  All these
methods apply asynchronous parallelism, so the time required by each
cell of the grid to perform the same number of training epochs varies.
Thus, we report the computational time of a run as the time required
by each independent run to return the best ensemble of generators found. 

\begin{table}[!h]
	\centering
	\small
	\caption{\small Computation time required by the evaluated GAN training methods in minutes.}
	\label{tab:computation-time}
\begin{tabular}{lrrrrr}
\toprule
\textbf{Method} &  \textbf{Mean}$\pm$\textbf{Std} &  \textbf{Median} &   \textbf{Iqr} &   \textbf{Min} &   \textbf{Max} \\
\midrule
\multicolumn{6}{c}{\textit{\xGrid{3}-Grid}} \\
\oppagan & 38.07$\pm$2.73 & 37.51 &  3.49 &  33.57  &  44.28 \\ 
\spagan & 87.20$\pm$0.31 & 87.15 &  0.34 &  86.72  &  88.02 \\
\nocommgan & 81.88$\pm$4.55 & 81.34 &  9.41 &  74.40  &  88.19 \\ 
\Lipi & 87.89$\pm$1.15 & 87.73 &  1.23 &  85.57  &  90.23 \\ 
\midrule
\multicolumn{6}{c}{\textit{\xGrid{4}-Grid}} \\
\spagan & 90.72$\pm$0.58 & 90.89 &  0.39 &  88.97  &  91.27 \\
\Lipi & 91.30$\pm$0.94 & 91.07 &  1.01 &  90.23  &  94.26 \\
\midrule
\multicolumn{6}{c}{\textit{\xGrid{5}-Grid}} \\
\spagan & 101.88$\pm$1.64 & 100.91 &  2.10 &  100.18  &  105.52 \\  
\Lipi & 105.64$\pm$3.25 & 107.22 &  4.48 &  100.25  &  111.05 \\ 
\bottomrule
\end{tabular}
\end{table}

The computational cost of \oppagan includes the time of training the GANs plus the time of optimizing the ensemble weights by using the ES-(1+1).
This method is the least computational cost method (see Table~\ref{tab:computation-time}). It trains a single network and there is not any communication among the different cells.

According to the Mann-Whitney U and posthoc statistical tests,
\Lipi requires the longest computation times.
It applies both, communication among the cells and selection/replacement in the sub-populations.

When comparing among \Lipi, \spagan, and \nocommgan,
the impact on the computation time of applying communication in \Lipi and \spagan is higher than the use of selection/replacement in \Lipi and \nocommgan (see Table~\ref{tab:computation-time} \textit{\xGrid{3}-Grid}). 
This increase in the computation cost may increase in problems that require the use and exchange among the cells bigger models (networks) for the generators and discriminators.

When analyzing the methods in which the cells exchange information, \Lipi and \spagan, 
the first one applies evaluates the networks in the cell by using a \textit{all-vs-all} pattern and 
\spagan uses \textit{one-vs-one} (see Section~\ref{sec:methods}).
The difference between their computation times grows with the grid size. 

Therefore, answering the \textbf{RQ3:} \textit{What is the impact on the computational cost of applying exchange of individuals and selection/replacement?}, the effect of applying selection/replacement is negligible when comparing it with the impact of 
communicating among the cells (copying the neighbors), when running the methods on \xGrid{3} grid. However, it increases as the grid size is larger. 
The importance of the communication may be larger when we use the same approach to train networks to address harder problems, and therefore, with much more parameters.  



==> gan-training.tex <==
\section{Background}
\label{sec:background}

This section introduces the main concepts in GANs training and
presents some related works dealing with robust GAN
training and distributed machine learning.

\subsection{General GAN training}
\label{sec:gan-training}

% TODO why not cite lipi instead?

In this study, we adopt the notation similar
to~\cite{arora2017generalization,li2017towards}.  Let $\calG=\{G_g, g
\in \calU\}$ and $\calD=\{D_d, d \in \calV\}$ denote the class of
generators and discriminators, where $G_g$ and $D_d$ are functions
parameterized by $g$ and $d$.  $\calU, \calV \subseteq \R^{p}$
represent the respective parameters space of the generators and
discriminators.  Finally, let $G_*$ be the target unknown distribution
to which we would like to fit our generative model.

Formally, the goal of GAN training is to find parameters $g$ and $d$
in order to optimize the objective function
\begin{equation}
\label{eq:gan-def}
\min_{g\in \calU}\max_{d \in \calV} \calL(g,d)\;, \;\text{where} \nonumber
\end{equation}
\begin{equation}
\calL(g,d) = \E_{x\sim G_*}[\phi (D_d(x))] + \E_{x\sim G_g}[\phi(1-D_d(x))]\;,
\end{equation}
and $\phi:[0,1] \to \R$, is a concave \emph{measuring function}.  In
practice, we have access to a finite number of training samples $x_1,
\ldots, x_m \sim G_*$.  Therefore, an empirical version
$\frac{1}{m}\sum_{i=1}^{m} \phi(D_d(x_i))$ is used to estimate
$\E_{x\sim G_*}[\phi (D_d(x))]$. The same also holds for $G_g$.

The methods analyzed in this study perform the same training by
addressing the optimization introduced in Eq.~\ref{eq:gan-def}.  They
apply stochastic gradient descent (SGD) based on binary cross-entropy
(BCE) loss (Eq.~\ref{eq:minmax-mut}). The main idea is to minimize the
Jensen–Shannon divergence (JSD) between the real ($p$) and fake ($q$)
data distributions, i.e., $JSD(p\parallel q)$. Eq.~\ref{eq:minmax-mut}
shows the loss function used to train the generators.
  \begin{align}
    \label{eq:minmax-mut}
    M^{BCE}_G &= \frac{1}{2} \E_{x\sim G_g}[log(1-D_d(x))]
  \end{align}  

\subsection{Related work}
\label{sec:related-work}

In 2014, Goodfellow described basic GAN
training~\cite{goodfellow2014generative}. Robust GAN training methods
is still investigated~\cite{arora2017generalization, li2017towards}.
Several practices that provided competitive results have been proposed
to stabilize the training~\cite{ganhacks}.  These methods include:
using different cost functions to the generator or
discriminator~\cite{arjovsky2017wasserstein,mao2017least,nguyen2017dual,zhao2016energy,
  wang2019evolutionary}; mitigating the impact of the learning rate
after a given number of iterations~\cite{radford2015unsupervised}; and
applying ensemble concepts~\cite{wang2016ensembles}.

\paragraph{Populations of GANs}
Some authors presented GAN training methods that involve multiple
generators and/or discriminators for improving robustness.  These
methods empirically show promising results.  Some examples are:
iteratively training and adding new generators with boosting
techniques~\cite{tolstikhin2017adagan}; combining a cascade of
GANs~\cite{wang2016ensembles}; training an array of discriminators on
a specific different low-dimensional projection of the
data~\cite{neyshabur2017stabilizing}; training the generator against a
dynamic ensemble of discriminators~\cite{mordido2018dropout};
independently optimizing several ``local'' generator-discriminator
pairs so that a ``global'' supervising pair of networks can be trained
against them~\cite{chavdarova2018sgan}.

\paragraph{Distributed Parallel Evolutionary Computing} 
Evolutionary algorithms (EAs) provide very competitive results dealing to hard-to-solve optimization problems. 
However, they show limited effectiveness and runtime for high dimensional problems~\cite{talbi2009metaheuristics}. 
Several authors proposed parallelism to deal with this limitation. This allows them to make problem instances tractable in practice and to keep computation times at reasonable levels~\cite{alba2013parallel}.
As in deep learning, the raising of GPUs is allowing the emergence of GPU based parallel EAs~\cite{essaid2019gpuea}. 

Here, we focus on a distributed cellular EA that intrduces the concept of ``neighborhood'', so that an individual may only interact with its nearby neighbors~\cite{alba2009cellular}. 
Each neighborhood (sub-population) evolves in parallel. 
The reduced size of the neighborhood fosters exploitation (faster convergence). 
The overlapped small neighborhood keeps diversity inside the sub-populations and helps in exploring the search space since a slow diffusion of solutions through the population provides a kind of exploration~\cite{alba2013parallel}. 

\paragraph{Distributed Evolutionary Machine Learning}
Some examples of scalable and large-scale evolutionary
computation systems are: EC-Star~\cite{hodjat2014maintenance}, which
runs on hundreds of desktop machines; a simplified version of Natural
Evolution Strategies~\cite{wierstra2008natural} with a novel
communication strategy to a collection of reinforcement learning
benchmark problems~\cite{salimans2017evolution} or deep convolutional
networks with over 4~million parameters trained with genetic
algorithms~\cite{clune2017uber}.

%% TODO we should talk more about selection pressure and communication in EC since they are our key study points, there must be some parallel EC work on this.

\paragraph{Spatial Distributed Evolutionary GAN Training}

In this study, we focus on spatially distributed evolutionary GAN
training. Theoretical studies and empirical results demonstrate that
the spatially distributed coevolutionary GAN training mitigates GAN
training problems (i.e., convergence
pathologies)~\cite{schmiedlechner2018towards,schmiedlechner2018lipizzaner,toutouh2019}.
\Lipi~\cite{schmiedlechner2018towards,schmiedlechner2018lipizzaner}
uses a spatial distributed competitive coevolutionary algorithm.  It
places the individuals of the generator and discriminator populations
on each cell of a spatial grid (i.e., each cell contains a pair of
generator-discriminator).  Overlapping Moore neighborhoods are defined
to allow communication among the different cells.  Each generator is
evaluated against all the discriminators of its neighborhood and the
same happen with each discriminator.  Besides, it takes advantage of
neighborhood communication to propagate models.  This type of GAN
training fosters diversity to address issues such as mode collapse.
Mustangs~\cite{toutouh2019} applies a similar approach but it
increases the diversity by applying different cost/loss functions in
each cell.  These two approaches return an ensemble/mixture of
generators defined by the neighborhood (sub-population of generators)
and the mixture weights that have shown competitive results on
standard benchmarks.

One concern with distributed evolutionary computing methods for
machine learning is the computation cost.  GANs training is costly and
training populations of them is challenging and even costlier.
Lipizzaner and Mustangs provide an asynchronous approach that can be
applied to train the different cells on a large-scale parallel
computation infrastructure, enabling scaling the training process.

In this study, we investigate the impact of two key components for
diversity in distributed coevolutionary GAN training methods like
Lipizzaner. The components we analyze are the communication among the
cells via the propagation of solutions through the grid, and the
application of the performance-based selection inside each
sub-population (cell). 







==> implementation.tex <==
\section{Methods implementation}
\label{sec:implementation}
This section summarizes the main aspects of the implementation of the three parallel methods studied in this research. 
\Lipi and \spagan are developed over open source MIT licensed. It is 
is written in \texttt{Python3} and uses \texttt{Pytorch}\footnote{Pythorch web site - \url{https://pytorch.org/}}.  
\texttt{Docker}\footnote{Docker web site - \url{https://www.docker.com/}} swarm and \texttt{docker-machine} is used to support distribution. 
The source is available from \url{https://github.com/mustang-gan/mustang/tree/master/mustang/src}. 

A master-client design model is used for communication. 
Clients are added by starting the application on more nodes, running pre-configured virtual machines, or with \texttt{Docker}. 

The master (or \emph{orchestrator}) is meant to control the whole training process. 
Its performs the following tasks: 
\begin{inparaenum}[\itshape 1)]
\item parsing the configuration, connecting to clients nodes, and transmiting the experiment configuration to all of them;
\item periodically checking client state, i.e. if the experiment has ended, or if the client may be not reachable anymore, unreachable clients can be ignored, or the entire experiment terminated;
\item gathering finished results, saving them to its disk, and ranking the final mixtures by their scores, e.g., FID. \end{inparaenum}

A modest computation power is required by the task overhead. 
The computation instances communicate with \textit{Hypertext Transfer Protocol} HTTP web services and exchange only relatively small amounts of data during the training process, 
it is possible to deploy multiple instances onto different machines and hence scale horizontally.

Each client node performs the computations of a sincle cell in the spatial grid. 
It starts by receiving the configuration parameters for the training process from the master. 
The client task can be summarized in three main steps:
\begin{inparaenum}[\itshape 1)]
	\item When a new experiment is requested, it parses the configuration file received and executes the specified training algorithm. It furthermore requests data from the neighboring cells each time the 	algorithm accesses the respective properties of the populations. 
If no experiment is running, the client runs in the background and listens for experiment requests on a specific port. 		
	\item It offers HTTP endpoints simultaneously to execute the training process. Other clients can also access these endpoints and request the current populations and optimizer parameters.
	\item The master actively monitors the clients and collects the
	results. After this, the client changes its state from \texttt{Busy}
	to \texttt{Idle} and waits for new experiment requests. 
\end{inparaenum}
